Cauchy problems for Einstein equations in three-dimensional spacetimes

We analyze existence and properties of solutions of two-dimensional general relativistic initial data sets with a negative cosmological constant, both on spacelike and characteristic surfaces. A new family of such vacuum, spacelike data parameterised by poles at the conformal boundary at infinity is constructed. We review the notions of global Hamiltonian charges, emphasising the difficulties arising in this dimension, both in a spacelike and characteristic setting. One or two, depending upon the topology, lower bounds for energy in terms of angular momentum, linear momentum, and center of mass are established.

==> macros.tex <==
{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{figure}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{table}{section}
\renewcommand{\thetable}{\thesection.\arabic{table}}

\newcommand{\h}{\red{h}}

\newcommand{\hone}{\blue{\stackrel{(1)}{\h}}}
\newcommand{\htwo}{\blue{\stackrel{(2)}{\h}}}

\newcommand{\tltwo}{\red{\ell}}


\newcommand{\hyp}{\blue{\mycal S}}

\newcommand{\Rg}{\blue{R_{g}}}
\newcommand{\Rtg}{\blue{R_{\tg}}}

\newcommand{\matter}{\red{\rho}}

\newcommand{\mc}{\red{m_c}}

\newcommand{\hL}{\blue{\hat L}}

\newcommand{\mzg}{\red{\mathring{g}}}

\newcommand{\zu}{\red{\mathring{u}}}

\newcommand{\ptcn}[1]{\ptc{#1}}

\newcommand{\mlambda}{\blue{\gamma}}
\newcommand{\bluecaref}{\mnote{change as requested by a referee}\color{teal} }
\newcommand{\bluecar}{\mnote{correction}\color{teal} }
\newcommand{\bluecad}{\mnote{addition}\color{teal} }

\newcommand{\gx}{ x}
\newcommand{\gz}{ z}
\newcommand{\gr}{ \rho}
\newcommand{\zg}{ \tg}
\newcommand{\zL}{ \tL}
\newcommand{\zK}{ \tK}
\newcommand{\Lpsikg}[2]{\mathring H_{\phi,\psi}^{#1}(#2)}
\newcommand{\Lpsik}[1]{\mathring H_{\phi,\psi}^{#1}}
\newcommand{\sources}{{\mycal C}}
\newcommand{\Ka}{ K_0}
\newcommand{\Kb}{ K_1}
\newcommand{\ga}{g_0}
\newcommand{\gb}{ g_1}

\newcommand{\fourb}{\blue{\mathbf{b}}}

\newcommand{\redc}{\color{red} }
\newcommand{\bluec}{\color{blue} }
\newcommand{\tealc}{\color{teal} }
\newcommand{\blueca}[1]{\color{blue} \ptc{changed or added on #1} }
%\newcommand{\bluecaraphaela}[1]{\color{blue} \rw{changed or added on #1} }
\newcommand{\ptchange}[1]{\color{blue} \ptc{changed on #1} }
\newcommand{\redca}[1]{\color{red}\mnote{ptc: added or changed on #1} }


\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\fuchsia}[1]{{\color{Fuchsia}#1}}
\newcommand{\jgreen}[1]{{\color{Junglegreen}#1}}
\newcommand{\mnblue}[1]{{\color{MidnightBlue}#1}}
\newcommand{\turquoise}[1]{{\color{Turquoise}#1}}
\newcommand{\dblue}[1]{{\color{Blue}#1}}


\newcounter{mnotecount}[section]

\renewcommand{\themnotecount}{\thesection.\arabic{mnotecount}}

\newcommand{\mnote}[1]%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
			$%\!\!\!\!\!\!\,
			\bullet$\themnotecount}}$ \marginpar{%\color{red}%
		\raggedright\tiny\em
		$\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }



\newcommand{\ptcr}[1]{{\color{red}\mnote{{\color{red}{\bf ptcr:}
				#1} }}}
\newcommand{\ptcrt}[1]{{\color{red}\mnotet{{\color{red}{\bf ptc:}
				#1} }}}
\newcommand{\ptct}[1]{{\mnotet{{\bf ptc:}
			#1} }}

\newcommand{\ptcb}[1]{{\color{blue}\mnote{{\color{blue}{\bf ptc:}
				#1} }}}
\newcommand{\ptcheck}[1]{{\color{blue}\mnote{{\color{blue}{\bf ptc checked on}
				#1} }}}



\newtheorem{theorem}{\sc  Theorem\rm}[section]
\newtheorem{acknowledgement}[theorem]{\sc  Acknowledgement\rm}
\newtheorem{algorithm}[theorem]{\sc  Algorithm\rm}
\newtheorem{axiom}[theorem]{\sc  Axiom\rm}
\newtheorem{Theorem}[theorem]{\sc  Theorem\rm}
\newtheorem{thm}[theorem]{\sc  Theorem\rm}
%\newtheorem{case}[theorem]{\sc  Case\rm}
\newtheorem{claim}[theorem]{\sc  Claim\rm}
\newtheorem{conclusion}[theorem]{\sc  Conclusion\rm}
\newtheorem{condition}[theorem]{\sc  Condition\rm}
\newtheorem{conjecture}[theorem]{\sc  Conjecture\rm}
\newtheorem{corollary}[theorem]{\sc  Corollary\rm}
\newtheorem{Corollary}[theorem]{\sc  Corollary\rm}
\newtheorem{criterion}[theorem]{\sc  Criterion\rm}
\newtheorem{definition}[theorem]{\sc  Definition\rm}
\newtheorem{lemma}[theorem]{\sc Lemma\rm}
\newtheorem{Lemma}[theorem]{\sc Lemma\rm}
\newtheorem{notation}[theorem]{\sc Notation\rm}
\newtheorem{problem}[theorem]{\sc Problem\rm}
\newtheorem{prop}[theorem]{\sc Proposition\rm}
\newtheorem{Proposition}[theorem]{\sc Proposition\rm}

\theorembodyfont{}

\newtheorem{example}[theorem]{\sc  Example\rm}
\newtheorem{exercise}[theorem]{\sc  Exercise\rm}

\newtheorem{remark}[theorem]{\sc Remark\rm}
\newtheorem{Remark}[theorem]{\sc Remark\rm}
\newtheorem{Remarks}[theorem]{\sc Remarks\rm}
\newtheorem{remarks}[theorem]{\sc Remarks\rm}
\newtheorem{solution}[theorem]{\sc Solution\rm}
\newtheorem{summary}[theorem]{\sc Summary\rm}


\newcommand{\begproof}{{\noindent\sc Proof:\ }}

\newcommand{\proof}{\begproof}
\newcommand{\eproof}{\blue{\hfill$\Box$}}
\newcommand{\eproofskip}{\blue{\hfill$\Box$}\medskip}
\newcommand{\qedskip}{\blue{\hfill$\Box$}\medskip}
\newcommand{\qed }{\blue{\hfill$\Box$}}
\newcommand{\ee}{\end{equation}}
\newcommand{\be}{\begin{equation}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\bel}[1]{\begin{equation}\label{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\eq}[1]{\eqref{#1}}
\newcommand{\eqrefl}[1]{\eqref{#1}}
\newcommand{\bth}{\begin{theorem}}
\newcommand{\eth}{\end{theorem}}
\newcommand{\bthl}[1]{\begin{theorem}\label{#1}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\bpropl}[1]{\begin{prop}\label{#1}}


\newcommand{\inv}{\blue{g}}

\newcommand{\btdv}{\blue{\tilde{\underline{u}}}}


\newcommand{\nmnM}{\red{{}^{n-1}M}}
\newcommand{\nuzero}{\red{\nu^0}}
\newcommand{\nuone}{\red{\nu_1}}
\newcommand{\nuz}{\red{\nu_v}}
\newcommand{\nuzup}{\red{\nu^u}}
\newcommand{\tdx}{\red{x}}%{\tilde x}
\newcommand{\tdv}{\red{\tilde v}}
\newcommand{\tdu}{\red{u}}%{\tilde u}
\newcommand{\tdr}{r}%{\tilde r}
\newcommand{\tdA}{A}%{\tilde A}
\newcommand{\tdB}{B}%{\tilde B}
\newcommand{\tdC}{C}%{\tilde C}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2} }
\newcommand{\tdD}{\tilde\nabla}
\newcommand{\snD}{\cancel\nabla}
\newcommand{\sng}{\cancel{g}}
\newcommand{\hkappafour}{ \hat{\kappa}_4}
\newcommand{\hkappafive}{ \hat{\kappa}_5}
\newcommand{\hkappatwo}{ \hat{\kappa}_2}
\newcommand{\Hf}{\blue{H}}
\newcommand{\Vf}{\blue{X}}
%\newcommand{\qh}{\blue{\hat q}}
\newcommand{\Lqh}{\blue{f}}
\newcommand{\hkappaone}{ \hat{\kappa}_1}
\newcommand{\hkappasix}{ \hat{\kappa}_6}
\newcommand{\hkappa}{\hat{\kappa}}
\newcommand{\opsi}{\overline{\psi}}
\newcommand{\ochi}{\red{\chi}}%{\overline\chi}
\newcommand{\ckappa}{\blue{ {\kappa}} }

\newcommand{\pt}[1]{\phantom{#1}}

\newcommand{\mtdell}{\blue{\check \ell}}%{\tilde x}
\newcommand{\mtdl}{\mtdell}%{\tilde x}
\newcommand{\mtdmu}{\blue{\check \mu}}%{\tilde x}
\newcommand{\mtdx}{\blue{\check x}}%{\tilde x}
\newcommand{\mtdg}{\blue{\check g}}%{\tilde x}
\newcommand{\mtdv}{\blue{\check v}}
\newcommand{\mtdu}{\blue{\check u}}%{\tilde u}
\newcommand{\mtdr}{\blue{\check r}}%{\tilde r}
\newcommand{\mtdA}{\blue{\check A}}%{\tilde A}
\newcommand{\mtdB}{\blue{\check B}}%{\tilde B}
\newcommand{\mtdC}{\blue{\check C}}%{\tilde C}
\newcommand{\mtdD}{\blue{\check D}}%{\tilde C}


 \newcommand{\ddim}{{\blue{d}}}
 \newcommand{\dmanif}{\blue{{}^\ddim M}}
 \newcommand{\dmetric}{{\blue{\mathring{\gamma}}}}
 \newcommand{\dnabla}{\blue{\mathring{D}}}
 \newcommand{\dDelta}{\blue{\Delta_{\dmetric}}}
 \newcommand{\dR}{\blue{\mathring{R}}}
 

\newcommand{\cell}{\blue{\check{\ell}}}
\newcommand{\cA}{\blue{\check{A}}}
\newcommand{\cB}{\blue{\check{B}}}
\newcommand{\cl}{\blue{\check{\ell}}}
\newcommand{\cu}{\blue{\check{u}}}
\newcommand{\cx}{\blue{\check{x}}}
\newcommand{\checkr}{\blue{\check{r}}}


\newcommand{\chmu}{\mtdmu}
\newcommand{\chx}{\mtdx}
\newcommand{\chell}{\mtdl}
\newcommand{\chl}{\mtdl}
\newcommand{\chg}{\mtdg}
\newcommand{\chv}{\mtdv}
\newcommand{\chu}{\mtdu}
\newcommand{\chr}{\mtdr}
\newcommand{\chA}{\mtdA}
\newcommand{\chB}{\mtdB}
\newcommand{\chC}{\mtdC}



\newcommand{\nur}{\blue{\nu_r}}


%%%Commandes:

%Ensembles:
\newcommand{\HP}{\mathcal{H}}

\newcommand{\B}{\red{D(0,1)}}%{\mathcal{B}}
\newcommand{\Bpr}{\red{D(p,r)}}%{\mathcal{B}}

\newcommand{\Bn}{\red{B(0,1)}}%{\mathcal{B}}
\newcommand{\Bnr}{\red{B(p,r)}}%{\mathcal{B}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Per}{\mathcal{P}_{2\pi}}
\newcommand{\Bxo}{B_{\rho_0}}
\newcommand{\bBxo}{\overline{B}_{\rho_0}}
\newcommand{\Cinf}[1]{C^\infty\left(#1\right)}
\newcommand{\Hc}[1]{H^2_0\left(#1\right)}

%Objets:
%Facteurs conformes
\newcommand{\qp}{{\red{\breve\phi}}}

%Opérateurs
\newcommand{\NL}{\fuchsia F}

\newcommand{\aL}{\mnblue L}
\newcommand{\aF}{\mnblue{\hat F}}
\newcommand{\aS}{\mnblue S}

%métrique physique
\newcommand{\pg}{\orange g}
\newcommand{\pK}{\orange K}
\newcommand{\pL}{\orange L}

\newcommand{\pJ}{\orange J}

%métrique plate
\newcommand{\qf}{\blue{\breve f}}
\newcommand{\qh}{\blue{h}}
\newcommand{\qhm}{\blue{h_\mu}}
\newcommand{\qL}{\blue{\breve{L}}}
\newcommand{\qD}{\blue{\breve{D}}}
\newcommand{\qg}{\blue{\breve g}}
\newcommand{\Lxx}{\qL_{\bx\bx}}
\newcommand{\Lxy}{\qL_{\bx\by}}
\newcommand{\qa}{\blue{a}}
\newcommand{\qb}{\blue{b}}
\newcommand{\qc}{\blue{c}}
\newcommand{\qpsi}{\blue{\breve\phi}}
\newcommand{\qpi}{\blue{\breve\pi}}
\newcommand{\q}[1]{\blue{\breve{#1}}}

%métrique hyperbolique: halfplane
\newcommand{\hg}{\hat{g}}

%métrique hyperbolique: disk
\newcommand{\tg}{\tilde{g}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tA}{\tilde{A}}

%métrique ADM
\newcommand{\ADMg}{\textbf{\pg}}

%Coordonnées:
%Demi-plan
\newcommand{\hx}{\dblue{\hat{x}}}
\newcommand{\hy}{\dblue{\hat{y}}}
\newcommand{\hht}{\dblue{\hat{t}}}
\newcommand{\hr}{\dblue{\hat{r}}}
\newcommand{\hz}{\dblue{\hat{z}}}
\newcommand{\hang}{\dblue{\hat\varphi}}

%Boule
\newcommand{\bcoord}{\textbf{y}}
\newcommand{\bx}{\red x}
\newcommand{\by}{\red y}
\newcommand{\br}{\red r}
\newcommand{\bz}{\red z}
\newcommand{\bang}{\red \theta}
\newcommand{\bro}{\red \omega}

\newcommand{\rr}{\red{r}}
\newcommand{\ptcnh}[1]{\ptc{#1}}

\newcommand{\tmcM}{\blue{\,\,\,\,\widetilde{\!\!\!\!\mcM}}}
\newcommand{\fourg}{\blue{\mathbf{g}}}
\newcommand{\mcM}{\mycal{M}}
\newcommand{\tfourg}{\blue{\widetilde{\fourg}}}

%Function Space
\newcommand{\df}{\blue{x}}
\newcommand{\Hkpp}{H^k_{\phi,\psi}}
\newcommand{\zHkpp}{\mathring H^k_{\phi,\psi}}
\newcommand{\zHk}{\mathring H^k}
\newcommand{\zH}{\mathring H}

%Raccourcis
\newcommand{\iju}[1]{#1^{ij}}
\newcommand{\ijd}[1]{#1_{ij}}
\newcommand{\mnu}[1]{#1^{\mu\nu}}
\newcommand{\mnd}[1]{#1_{\mu\nu}}
\newcommand{\norm}[2]{\left| #1 \right|_{#2}}
\newcommand{\normsq}[2]{| #1 |_{#2}^{2}}
\newcommand{\normf}[2]{\lVert #1 \rVert_{#2}}
\newcommand{\normfsq}[2]{\lVert #1 \rVert_{#2}^{2}}
\newcommand{\ov}{\overline}
\newcommand{\gO}[1]{O\big(#1\big)}%{\mathcal{O}\left(#1\right)}

\newcommand{\MyPsi}{\red{\phi}}
\newcommand{\myPsi}{\blue{\MyPsi}}
\newcommand{\mypsi}{\myPsi}
\newcommand{\tmyPsi}{{\MyPsi}}

\newcommand{\defining}{\red{\omega}}

%Commentaires:
\newcommand{\ptc}[1]{\mnote{{\bf ptc:}#1}}

\newcommand{\tqn}[1]{\mnote{{\bf tq:}#1}}


\DeclareFontFamily{OT1}{rsfs}{}
\DeclareFontShape{OT1}{rsfs}{m}{n}{ <-7> rsfs5 <7-10> rsfs7 <10-> rsfs10}{}
\DeclareMathAlphabet{\mycal}{OT1}{rsfs}{m}{n}

%Perso
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\loc}{loc}
\newcommand{\iset}[2]{[\![#1,#2]\!]}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% RENEW COMMANDS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% WITHOUT COLORS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







\renewcommand{\Rg}{R_{g}}
\renewcommand{\Rtg}{R_{\tg}}
\renewcommand{\matter}{\rho}
\renewcommand{\mc}{m_c}
\renewcommand{\mzg}{\mathring{g}}
\renewcommand{\zu}{\mathring{u}}
\renewcommand{\mlambda}{\gamma}
\renewcommand{\fourb}{\mathbf{b}}


\renewcommand{\eproof}{{\hfill$\Box$}}
\renewcommand{\eproofskip}{{\hfill$\Box$}\medskip}
\renewcommand{\qedskip}{{\hfill$\Box$}\medskip}
\renewcommand{\qed }{\hfill$\Box$}


\renewcommand{\inv}{{g}}
\renewcommand{\btdv}{{\tilde{\underline{u}}}}
\renewcommand{\nmnM}{{{}^{n-1}M}}
\renewcommand{\nuzero}{{\nu^0}}
\renewcommand{\nuone}{{\nu_1}}
\renewcommand{\nuz}{{\nu_v}}
\renewcommand{\nuzup}{{\nu^u}}
\renewcommand{\tdx}{{x}}%{\tilde x}
\renewcommand{\tdv}{{\tilde v}}
\renewcommand{\tdu}{{u}}%{\tilde u}

\renewcommand{\Hf}{ {H}}
\renewcommand{\Vf}{ {X}}
\renewcommand{\Lqh}{ {f}}

\renewcommand{\ochi}{{\chi}}%{\overline\chi}
\renewcommand{\ckappa}{ { {\kappa}} }

\renewcommand{\mtdell}{ {\check \ell}}%{\tilde x}
\renewcommand{\mtdmu}{ {\check \mu}}%{\tilde x}
\renewcommand{\mtdx}{ {\check x}}%{\tilde x}
\renewcommand{\mtdg}{ {\check g}}%{\tilde x}
\renewcommand{\mtdv}{ {\check v}}
\renewcommand{\mtdu}{ {\check u}}%{\tilde u}
\renewcommand{\mtdr}{ {\check r}}%{\tilde r}
\renewcommand{\mtdA}{ {\check A}}%{\tilde A}
\renewcommand{\mtdB}{ {\check B}}%{\tilde B}
\renewcommand{\mtdC}{ {\check C}}%{\tilde C}
\renewcommand{\mtdD}{ {\check D}}%{\tilde C}


\renewcommand{\ddim}{{ {d}}}
\renewcommand{\dmanif}{ {{}^\ddim M}}
\renewcommand{\dmetric}{{ {\mathring{\gamma}}}}
\renewcommand{\dnabla}{ {\mathring{D}}}
\renewcommand{\dDelta}{ {\Delta_{\dmetric}}}
\renewcommand{\dR}{ {\mathring{R}}}


\renewcommand{\cell}{ {\check{\ell}}}
\renewcommand{\cA}{ {\check{A}}}
\renewcommand{\cB}{ {\check{B}}}
\renewcommand{\cl}{ {\check{\ell}}}
\renewcommand{\cu}{ {\check{u}}}
\renewcommand{\cx}{ {\check{x}}}
\renewcommand{\checkr}{ {\check{r}}}

\renewcommand{\nur}{ {\nu_r}}


\renewcommand{\B}{{D(0,1)}}%{\mathcal{B}}
\renewcommand{\Bpr}{{D(p,r)}}%{\mathcal{B}}

\renewcommand{\Bn}{{B(0,1)}}%{\mathcal{B}}
\renewcommand{\Bnr}{{B(p,r)}}%{\mathcal{B}}

\renewcommand{\qp}{{{\breve\phi}}}

%Opérateurs
\renewcommand{\NL}{F}

\renewcommand{\aL}{ L}
\renewcommand{\aF}{{\hat F}}
\renewcommand{\aS}{ S}

%métrique physique
\renewcommand{\pg}{g}
\renewcommand{\pK}{K}
\renewcommand{\pL}{L}

\renewcommand{\pJ}{J}

%métrique plate
\renewcommand{\qf}{ {\breve f}}
\renewcommand{\qh}{ {h}}
\renewcommand{\qhm}{ {h_\mu}}
\renewcommand{\qL}{ {\breve{L}}}
\renewcommand{\qD}{{\breve{D}}}
\renewcommand{\qg}{{\breve g}}
\renewcommand{\Lxx}{\qL_{\bx\bx}}
\renewcommand{\Lxy}{\qL_{\bx\by}}
\renewcommand{\qa}{{a}}
\renewcommand{\qb}{{b}}
\renewcommand{\qc}{{c}}
\renewcommand{\qpsi}{{\breve\phi}}
\renewcommand{\qpi}{{\breve\pi}}
\renewcommand{\q}[1]{{\breve{#1}}}

%Coordonnées:
%Demi-plan
\renewcommand{\hx}{{\hat{x}}}
\renewcommand{\hy}{{\hat{y}}}
\renewcommand{\hht}{{\hat{t}}}
\renewcommand{\hr}{{\hat{r}}}
\renewcommand{\hz}{{\hat{z}}}
\renewcommand{\hang}{{\hat\varphi}}

\renewcommand{\bx}{ x}
\renewcommand{\by}{ y}
\renewcommand{\br}{ r}
\renewcommand{\bz}{ z}
\renewcommand{\bang}{ \theta}
\renewcommand{\bro}{ \omega}

\renewcommand{\rr}{{r}}
\renewcommand{\ptcnh}[1]{\ptc{#1}}

\renewcommand{\tmcM}{{\,\,\,\,\widetilde{\!\!\!\!\mcM}}}
\renewcommand{\fourg}{{\mathbf{g}}}
\renewcommand{\mcM}{\mycal{M}}
\renewcommand{\tfourg}{{\widetilde{\fourg}}}

%Function Space
\renewcommand{\df}{{x}}

%Raccourcis

\renewcommand{\MyPsi}{{\phi}}
\renewcommand{\myPsi}{{\MyPsi}}
\renewcommand{\mypsi}{\myPsi}
\renewcommand{\tmyPsi}{{\MyPsi}}

\renewcommand{\defining}{{\omega}}

